Exploring Frequency-Inspired Optimization in Transformer for Efficient Single Image Super-Resolution

Transformer-based methods have exhibited remarkable potential in single image super-resolution (SISR) by effectively extracting long-range dependencies. However, most of the current research in this area has prioritized the design of transformer blocks to capture global information, while overlooking the importance of incorporating high-frequency priors, which we believe could be beneficial. In our study, we conducted a series of experiments and found that transformer structures are more adept at capturing low-frequency information, but have limited capacity in constructing high-frequency representations when compared to their convolutional counterparts. Our proposed solution, the cross-refinement adaptive feature modulation transformer (CRAFT), integrates the strengths of both convolutional and transformer structures. It comprises three key components: the high-frequency enhancement residual block (HFERB) for extracting high-frequency information, the shift rectangle window attention block (SRWAB) for capturing global information, and the hybrid fusion block (HFB) for refining the global representation. To tackle the inherent intricacies of transformer structures, we introduce a frequency-guided post-training quantization (PTQ) method aimed at enhancing CRAFT's efficiency. These strategies incorporate adaptive dual clipping and boundary refinement. To further amplify the versatility of our proposed approach, we extend our PTQ strategy to function as a general quantization method for transformer-based SISR techniques. Our experimental findings showcase CRAFT's superiority over current state-of-the-art methods, both in full-precision and quantization scenarios. These results underscore the efficacy and universality of our PTQ strategy. The source code is available at: https://github.com/AVC2-UESTC/Frequency-Inspired-Optimization-for-EfficientSR.git.

==> tables/ab_modules.tex <==
\begin{table}[!t]
  \caption{Study of HFERB, SRWAB, and HFB on SISR. The results ($\times 4$) are obtained from the Manga109 dataset.}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{1.5mm}
  \begin{tabular}{cccccc}
      \toprule
      Model & HFERB & SRWAB & HFB & Concat & PSNR \\
      \midrule
      CRAFT$_{conv}$ & $\checkmark$ & & $\checkmark$ &  & 30.79\\
      CRAFT$_{tranformer}$ &  & $\checkmark$ & $\checkmark$ &  & 31.12 \\
      CRAFT$_{concat}$ & $\checkmark$ & $\checkmark$ &  & $\checkmark$ & 30.92\\
      CRAFT & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & 31.18\\
      \bottomrule
  \end{tabular}
  \label{tab:ablationmodules}
\end{table}

==> tables/ab_priors.tex <==
\begin{table}[!t]
  \caption{Effectiveness of high-frequency prior. The results ($\times 4$) are obtained from the Manga109 dataset.}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{2mm}
  \begin{tabular}{cccccc}
      \toprule
      Model & Regular & Swap & Cascade & PSNR & SSIM \\
      \midrule
      CRAFT$_{swap}$ &  & $\checkmark$ & & 30.67 & 0.9113\\
      CRAFT$_{cascade}$ &  & & $\checkmark$ & 30.88 & 0.9141\\
      CRAFT & $\checkmark$ & & & 31.18 & 0.9168\\
      \bottomrule
  \end{tabular}
  \label{tab:ablationcrs}
\end{table}

==> tables/sr_results.tex <==
\begin{table*}[!t]
  \caption{Performance comparison of different SISR models on five benchmarks. Params represents the total number of network parameters. Results for the best and second best candidates are \textbf{highlighted}, and \underline{underlined}.}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{3.2mm}
  \begin{tabular}{|c|c|c|c|c|c|c|c|}
      \hline
      Scale & Model & Params & \makecell[c]{Set5\\(PSNR/SSIM)} & \makecell[c]{Set14\\(PSNR/SSIM)} & \makecell[c]{BSD100\\(PSNR/SSIM)} & \makecell[c]{Urban100\\(PSNR/SSIM)} & \makecell[c]{Manga109\\(PSNR/SSIM)}\\
      \hline
      \multirow{11}{*}{${\times 4}$} & EDSR-baseline \cite{Lim2017} & 1518K & 32.09/0.8938 & 28.58/0.7813 & 27.57/0.7357 & 26.04/0.7849 & 30.35/0.9067\\
      & CARN \cite{Ahn2018} & 1592K & 32.13/0.8937 & 28.60/0.7806 & 27.58/0.7349 & 26.07/0.7837 & 30.47/0.9084\\
      & IMDN \cite{Hui2019} & 715K & 32.21/0.8948 & 28.58/0.7811 & 27.56/0.7353 & 26.04/0.7838 & 30.45/0.9075\\
      & LatticeNet \cite{luo2020latticenet} & 777K & 32.18/0.8943 & 28.61/0.7812 & 27.57/0.7355 & 26.14/0.7844 & -/-\\
      & LAPAR-A \cite{Li2020} & 659k & 32.15/0.8944 & 28.61/0.7818 & 27.61/0.7366 & 26.14/0.7871 & 30.42/0.9074\\
      & HPUN-L \cite{sun2022hybrid} & 734K & 32.31/0.8962 & 28.73/0.7842 & 27.66/0.7386 & 26.27/0.7918 & 30.77/0.9109\\
      \cdashline{2-8}[1pt/1pt]
      & SwinIR-light \cite{liang2021swinir} & 897K & \underline{32.44}/\underline{0.8976} & 28.77/0.7858 & \underline{27.69}/\underline{0.7406} & 26.47/0.7980 & \underline{30.92}/\underline{0.9151}\\
      & LBNet \cite{gao2022lightweight} & 742K & 32.29/0.8960 & 28.68/0.7832 & 27.62/0.7382 & 26.27/0.7906 & 30.76/0.9111\\
      & ESRT \cite{lu2022transformer} & 751K & 32.19/0.8947 & 28.69/0.7833 & \underline{27.69}/0.7379 & 26.39/0.7962 & 30.75/0.9100\\
      & ELAN-light \cite{zhang2022efficient} & 601K & 32.43/0.8975 & \underline{28.78}/\underline{0.7858} & \underline{27.69}/\underline{0.7406} & \underline{26.54}/\underline{0.7982} & \underline{30.92}/0.9150\\
      & CRAFT (Ours) & 753K & \textbf{32.52}/\textbf{0.8989} & \textbf{28.85}/\textbf{0.7872} & \textbf{27.72}/\textbf{0.7418} & \textbf{26.56}/\textbf{0.7995} & \textbf{31.18}/\textbf{0.9168}\\
      \hline
  \end{tabular}
  \label{tab:resultsLightweight}
\end{table*}
